Last-iterate Convergence in Extensive-Form Games

Regret-based algorithms are highly efficient at finding approximate Nash equilibria in sequential games such as poker games. However, most regret-based algorithms, including counterfactual regret minimization (CFR) and its variants, rely on iterate averaging to achieve convergence. Inspired by recent advances on last-iterate convergence of optimistic algorithms in zero-sum normal-form games, we study this phenomenon in sequential games, and provide a comprehensive study of last-iterate convergence for zero-sum extensive-form games with perfect recall (EFGs), using various optimistic regret-minimization algorithms over treeplexes. This includes algorithms using the vanilla entropy or squared Euclidean norm regularizers, as well as their dilated versions which admit more efficient implementation. In contrast to CFR, we show that all of these algorithms enjoy last-iterate convergence, with some of them even converging exponentially fast. We also provide experiments to further support our theoretical results.

==> efg.tex <==
\section{Definitions and Properties of Extensive-form Game with Imperfect Information} \label{sec: efg definition}

In this section, we follow most definitions from \citep{nisan2007algorithmic}.
A Extensive-form game with imperfect information is defined on a game tree.
We denote the collection of \emph{information sets} by $\csimp$, which is a partition of the nonterminal nodes in the tree. 
Each information set is a decision node for either $\x$ player or $\y$ player.
We use $\infoX$ and $\infoY$ to denote the set of the decision nodes for $\x$ player and $\y$ player, respectively. 
We also denote the set of terminal nodes by $\trmnl$.
Let $\cst$ be the cost vector for $\x$ player over $\trmnl$, which is also the utility of $\y$ player in zero-sum games.
Let $\actn$ be the set of action and $\actn_g$ be the set of actions for information set $g\in\csimp$.
%Without loss of generality, we assume $|\calA_h|>1$ for 
The set of pure actions for $\x$ player is $\prod_{g\in\infoX}\actn_g$ and a mixed strategy is a probability distribution over it.
The case is similar for $\y$. 

A \emph{sequence} of actions of a player is the sequence of his actions disregarding the actions of the other players on the unique path from the root to some node $e$ in the tree, denoted by $\seq(e)$.
We use $\emp$ to denote the empty sequence.
We define the game has \emph{perfect recall} if $\seq(s)=\seq(e)$ for any nodes $s,e\in g$, $g\in\csimp$.
In this case we define $\seq(g)\triangleq\seq(e)$ for any node $e\in g$.
We denote $\seqX\triangleq\{\emp\}\cup\{\seq(g)a\mid g\in\csimp^\x,~a\in\actn_h\}$ to be the set of sequences for $\x$ player.
We also define $\seqY$ similarly and let $\seqZ=\seqX\cup\seqY$.
For a nonterminal sequence $i$, we define $\csimp_i$ to be $\{g:g\in\csimp,\sigma(g)=i\}$, the collection of successive information sets following $i$.
We denote $h(i)$ to be the information set in the end of sequence $i$ starting from the root.
We will simply write $h$ when there is no confusion which sequence $i$ we deal with.

Given $i\in\seqX$, we define $x_i$, the \emph{realization probability} of $i$ for a mixed strategy for $\x$ player to be the probability that the strategy prescribes $i$.
Clearly, we have always $x_i\ge 0$ and 
\begin{align}
	x_{\emp}=1,\qquad\sum_{a\in\actn_g}x_{\seq(g)a}=x_{\seq(g)},~ \forall g\in\infoX. \label{eq: sequence form constraints}
\end{align}
%A well-known result (Kuhn's theorem) is that in perfect recall game, 
Similarly, we can define $y_j$ to be the {realization probability} of sequence $j$ for a mixed strategy for $\y$ player.
We denote the set of all feasible realization probabilities for $\x$ and $\y$ by $\treeX$ and $\treeY$, respectively.
The sequence for payoff matrix $\G\in\R^{|\seqX|\times|\seqY|}$
For $\sigma\in\seqX$ and $\tau\in\seqY$, we have
\begin{align*}
	G_{\sigma\tau}=\sum_{e\in\trmnl}c_{t}\cdot\one\{\text{$e$ is reached when the players play $\sigma$ and $\tau$}\}.
\end{align*}
In other word, the entry is nonzero only if both $\sigma$ and $\tau$ are terminal sequences. 
We can also write the linear constraints in \pref{eq: sequence form constraints} as a constraint matrix $\matX\in\R^{(|\infoX|+1)\times|\seqX|}$ such that a realization plan $\x\in\R^{|\seqX|}$ is valid if and only if
\begin{align*}
	\matX \x=\ve,~\x\ge \zero,
\end{align*}
where entries in $\ve$ are zero except for the first entry, indicating $x_{\emp}=1$.
Similarly for $\y$ player, we have the constraint matrix $\matY$ and vector $\vf$.
Consequently, we write the best response of $\x$ to a fixed $\y$ to as the following linear program:
\begin{align*}
	\min_{\x} \x^\top(\G\y),~\text{subject to}~\matX\x=\ve,~\x\ge \zero.
\end{align*}
The dual with variables $\bv\in\R^{|\infoX|+1}$ of this linear program is
\begin{align*}
	\max_{\bv} \ve^\top\bv,~\text{subject to}~\matX^\top \bv\le\G\y.
\end{align*}
On the other hand, $\y$ tries to maximize $\x^\top\G\y$, that is, maximize $\ve^\top\bv$ by strong duality.
Therefore, a maximin realization play $\y$ is a solution to 
\begin{align*}
	\max_{\bv,\y} \ve^\top\bv,~\text{subject to}~\matX^\top \bv\le\G\y,~\matY\y=\vf,~\y\ge\zero,
\end{align*}
which is also a linear program.
The dual of this linear problem is 
\begin{align*}
	\min_{\bu,\x} \vf^\top\bu,~\text{subject to}~\matY^\top \bu\ge\G^\top\x,~\matX\x=\ve,~\x\ge\zero.
\end{align*}
A solution to this dual is a minimax realization plan $\x$.
We assume there exists a unique optimal solution pair $\x^*,\y^*$ along with $\bv^*,\bu^*$.
By the complementary slackness, we have some slackness variables $\w^*\in\R^{|\seqX|},\s^*\in\R^{|\seqY|}$ such that $\x^*\odot\w^*=\zero$, $\y^*\odot\s^*=\zero$, and
\begin{align}\label{eq: complementary slackness}
\matX^\top \bv^*-\G\y^*+\w^*=\zero,\quad\matY^\top \bu^*-\G^\top\x^*-s^*=\zero,\quad\w^*,\s^*\geq\zero.
\end{align}
Moreover, the \emph{strict complementary slackness} (see, for example,~\citep[Theorem 10.7]{vanderbei2001linear}) ensures that besides \pref{eq: complementary slackness}, there exists an optimal solution (must be $(\x^*,\y^*)$ by our assumption) such that
\begin{align}\label{eq: strict complementary slackness}
	\x^*+\w^*>\zero,\quad\y^*+\s^*>\zero.
\end{align}
Note that \pref{eq: complementary slackness} and \pref{eq: strict complementary slackness} imply that for nonterminal sequence $i\in\seqX$, if $x^*_i>0$, we get
%\footnote{otherwise, we have more than one realization probabilities mapping to the same optimal mixed strategy by the assumption that $|\actn_h|>1$ for all $h\in\csimp$, violating the uniqueness assumption.}
\begin{align}\label{eq: value recursion optimal}
	\bv^*_\infoi-\sum_{g\in\csimp_i}\bv^*_g=(\matX^\top\bv^*)_i=(\matX^\top\bv^*-\G\y^*)_i=-w^*_i=0;
\end{align}
otherwise, if $x^*_i=0$, we have 
\begin{align}\label{eq: value recursion suboptimal}
	\bv^*_\infoi<\sum_{g\in\csimp_i}\bv^*_g.
\end{align}
Additionally, for terminal sequence $i$, we have
\begin{align*}
	\bv^*_\infoi=(\G\y^*)_i,~\text{for $i$ such that $x_i>0$, and }~\bv^*_\infoi<(\G\y^*)_i,~\text{otherwise.}
\end{align*}
The case is similar for $\bu^*$ and $\G^\top\x^*$.
Denoting ${\xterm}^*$ and ${\yterm}^*$ and the entries of $\x^*$ and $\y^*$ restricted on terminal sequences, we summary the results in the following lemma.
\begin{lemma}\label{lem: gap lemma}
    Given sequence $i$, we use $h$ to denote the information set that the last action of $i$ is in.
	We have
     \begin{align*}
		(\G\y^*)_i &= \bv^*_\infoi  &&\forall i\in \supp(\xterm^*), \\
		(\G\y^*)_i &> \bv^*_\infoi  &&\forall i\notin \supp(\xterm^*), \\
		(\G^\top\x^*)_i &= \bv^*_\infoi  &&\forall i\in\supp(\yterm^*), \\
		(\G^\top\x^*)_i &< \bv^*_\infoi &&\forall i\notin\supp(\yterm^*).
     \end{align*}
\end{lemma}
Therefore, the following problem-dependent constant $\xi$ is well-defined. 
\begin{definition}\label{def: xi}
    Given sequence $i$, we use $h$ to denote the information set that the last action of $i$ is in.
	We define
	\begin{align*}
    \xi\triangleq \min\left\{ \min_{i\notin\supp(\xterm^*)} (\G\y^*)_i - \bv^*_{\infoi}, \quad  \min_{i\notin\supp(\yterm^*)} \bv^*_{\infoi} -(\G^\top\x^*)_i \right\} \in (0,\diam]. 
    \end{align*}
\end{definition}

